Facial Expression Restoration Based on Improved Graph Convolutional Networks

Facial expression analysis in the wild is challenging when the facial image is with low resolution or partial occlusion. Considering the correlations among different facial local regions under different facial expressions, this paper proposes a novel facial expression restoration method based on generative adversarial network by integrating an improved graph convolutional network (IGCN) and region relation modeling block (RRMB). Unlike conventional graph convolutional networks taking vectors as input features, IGCN can use tensors of face patches as inputs. It is better to retain the structure information of face patches. The proposed RRMB is designed to address facial generative tasks including inpainting and super-resolution with facial action units detection, which aims to restore facial expression as the ground-truth. Extensive experiments conducted on BP4D and DISFA benchmarks demonstrate the effectiveness of our proposed method through quantitative and qualitative evaluations.

==> pdf_tex/igcn.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.6]{pdf/IGCN.pdf}
    \caption{Structure of the Improved Graph Convolutional Network $8*8$ with stride $1$. $Adj_{(i,j)}$ represents the link between $i$-th patch and $j$-th patch, $Adj$ represents adjacency matrix.  } 
    \label{fig:igcn}
\vspace{-3mm}
\end{figure}

==> pdf_tex/rrb.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.6]{pdf/RRB.pdf}
    \caption{Structure of Region Relation Modeling Block (RRMB), which consists of IGCN $1*1$, $2*2$, $8*8$. $1*1$ represents splitting only 1 patch for the inputs, $2*2$ represents splitting 4 patches for the inputs, and $8*8$ represents splitting 64 patches for the inputs.} 
    \label{fig:rrb}
\vspace{-3mm}
\end{figure}

==> table/mm.tex <==
\begin{table*}[!t]
\centering
\caption{F1-score and accuracy for 8 AUs on DISFA. Ours is the total loss to learn the proposed model, ours- lacks the loss of AUs classifier.}
%\scriptsize
\vspace{1mm}
\scalebox{0.73}{
\begin{tabular}{c|c|c  c  c  c  c}
\hline

Dataset & Feature & FGM & BIM-a & BIM-b & JSMA & Opt  \\ \hline
% 0.214	0.185	0.217	0.348	0.365	0.558	0.765	0.504	0.3945
\multirow{4}{*}{MNIST}
 &$0.107$  &$0.217$  &$0.214$    &$0.219$  &$0.901$  &$0.863$  \\
 &$0.010$  &$0.159$  &$0.185$    &$0.198$  &$0.958$  &$0.806$  \\
 &$0.091$  &$0.202$  &$0.217$    &$0.286$  &$0.739$  &$0.739$   \\
 &$0.392$  &$0.336$  &$0.348$    &$0.362$  &$0.870$  &$0.797$   \\ \hline
\multirow{4}{*}{CIFAR-10} 
 &$0.039$  &$0.185$  &$0.365$    &$0.270$  &$0.903$  &$0.945$   \\
 &$0.576$  &$0.548$  &$0.558$    &$0.628$  &$0.763$  &$0.741$   \\
 &$0.509$  &$0.654$  &$0.765$    &$0.746$  &$0.608$  &$0.809$   \\
 &$0.270$  &$0.506$  &$0.504$    &$0.524$  &$0.685$  &$0.725$   \\ \hline
\multirow{4}{*}{SVHN} 
 &$0.270$  &$0.506$  &$0.504$    &$0.524$  &$0.685$  &$0.725$   \\
 &$0.270$  &$0.506$  &$0.504$    &$0.524$  &$0.685$  &$0.725$   \\
 &$0.270$  &$0.506$  &$0.504$    &$0.524$  &$0.685$  &$0.725$   \\
 &$0.270$  &$0.506$  &$0.504$    &$0.524$  &$0.685$  &$0.725$   \\ \hine

\end{tabular}}
\label{tb:disfa}
\vspace{-3mm}
\end{table*}

